Hands Off: A Handshake Interaction Detection and Localization Model for COVID-19 Threat Control

The COVID-19 outbreak has affected millions of people across the globe and is continuing to spread at a drastic scale. Out of the numerous steps taken to control the spread of the virus, social distancing has been a crucial and effective practice. However, recent reports of social distancing violations suggest the need for non-intrusive detection techniques to ensure safety in public spaces. In this paper, a real-time detection model is proposed to identify handshake interactions in a range of realistic scenarios with multiple people in the scene and also detect multiple interactions in a single frame. This is the first work that performs dyadic interaction localization in a multi-person setting. The efficacy of the proposed model was evaluated across two different datasets on more than 3200 frames, thus enabling a robust localization model in different environments. The proposed model is the first dyadic interaction localizer in a multi-person setting, which enables it to be used in public spaces to identify handshake interactions and thereby identify and mitigate COVID-19 transmission.

==> image_page.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%
%%% This is placed here to get it in the right place when compiled
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \centering
     \captionsetup[subfigure]{aboveskip=2pt, belowskip=2pt}
     
     \begin{subfigure}[t]{0.48\textwidth}
        \includegraphics[width=\textwidth]{images/res-deee-shake-rand1.pdf}
        \caption{}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \includegraphics[width=\textwidth]{images/res-deee-fake1.pdf}
        \caption{Fake handshake by occlusion.}
        \label{fig:fakeshake}
    \end{subfigure}

    \caption{Detection localizations in busy settings and occlusion cases.}
    \label{fig:res-rand-shakes}
\end{figure*}
% \newpage

\begin{figure*}[b]
    \centering
    \captionsetup[subfigure]{aboveskip=2pt, belowskip=2pt}
    
    \begin{subfigure}{\columnwidth}
        \includegraphics[height=5cm,width=\textwidth]{images/res-uti-fail3.pdf}
        \caption{}
    \end{subfigure}
    %
    \hfill
    \begin{subfigure}{\columnwidth}
        \includegraphics[height=5cm,width=\textwidth]{images/res-uti-fail4.pdf}
        \caption{}
    \end{subfigure}
    %
    \hfill
    \begin{subfigure}{\columnwidth}
        \includegraphics[width=\textwidth]{images/res-deee-fail1.pdf}
        \caption{}
    \end{subfigure}
    %
    \hfill
    \begin{subfigure}{\columnwidth}
        \includegraphics[width=\textwidth]{images/res-deee-fail2.pdf}
        \caption{}
    \end{subfigure}
    %
    \hfill
    \begin{subfigure}{\columnwidth}
        \includegraphics[width=\textwidth]{images/res-deee-fail3.pdf}
        \caption{}
    \end{subfigure}
    %
    \hfill
    \begin{subfigure}{\columnwidth}
        \includegraphics[width=\textwidth]{images/res-deee-shakefail1.pdf}
        \caption{}
        \label{fig:deee-shakefail}
    \end{subfigure}
    %
    \caption{Localization false positives and false negatives in the model.}
    \label{fig:shakefails}
\end{figure*}


==> img_page2.tex <==
\begin{figure}[tbh]
    \centering
    \captionsetup[subfigure]{aboveskip=3pt, belowskip=3pt}
    
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[height=6.6cm,width=\textwidth]{images/PvsR_UTI.png}
        \caption{UTI dataset}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[height=6.6cm,width=\textwidth]{images/PvsR_DEEE.png}
        \caption{Shakes dataset}
    \end{subfigure}
\caption{Precision vs Recall curves for handshake localizer for UTI and Shakes dataset.}
\label{fig:PvsR_shake}
\end{figure}
\vspace{0.5cm}

\begin{figure}[tbh]
    \centering
    \captionsetup[subfigure]{aboveskip=2pt, belowskip=2pt}
    
    \begin{subfigure}[t]{\columnwidth}
        \includegraphics[width=\textwidth]{images/res-uti-shake1.pdf}
        \caption{UTI dataset frame}
        \label{fig:uti-shake1}
    \end{subfigure}%
    
    \begin{subfigure}[t]{\columnwidth}
        \includegraphics[height=5.2cm,width=\textwidth]{images/res-deee-shake2.pdf}
        \caption{Shakes dataset - two handshakes.}
        \label{fig:deee-2shakes}
    \end{subfigure}%
    
    \begin{subfigure}[t]{\columnwidth}
        \includegraphics[height=5.2cm,width=\textwidth]{images/res-deee-shake3.pdf}
        \caption{Handshakes at different distances from the camera.}
        \label{fig:deee-2shakes-scale}
    \end{subfigure}%
    
    \caption{Handshake interaction detection localizations.}
    \label{fig:res-shakes}
\end{figure}

